Active Sensing with Predictive Coding and Uncertainty Minimization

We present an end-to-end procedure for embodied exploration inspired by two biological computations: predictive coding and uncertainty minimization. The procedure can be applied to exploration settings in a task-independent and intrinsically driven manner. We first demonstrate our approach in a maze navigation task and show that it can discover the underlying transition distributions and spatial features of the environment. Second, we apply our model to a more complex active vision task, where an agent actively samples its visual environment to gather information. We show that our model builds unsupervised representations through exploration that allow it to efficiently categorize visual scenes. We further show that using these representations for downstream classification leads to superior data efficiency and learning speed compared to other baselines while maintaining lower parameter complexity. Finally, the modularity of our model allows us to probe its internal mechanisms and analyze the interaction between perception and action during exploration.

==> background.tex <==
In this section, we describe the theory of predictive coding, which underlies the perception component of our model. We also describe the connection between this theory and the framework of variational autoencoders in deep learning \cite{pred_theories, marino_pc_vae}. 
\subsection{Hierarchical Predictive Coding}
An important feature of the mammalian visual system is its hierarchical structure. Predictive coding \cite{rao_ballard} is a theory of sensory processing that views neural responses as latent states in a hierarchical generative model maintained by the brain. The neural responses at each level in the hierarchy are predicted by the responses at the level above, and the sensory input is predicted by the responses at the lowest level. According to predictive coding, the goal of perception is to infer these neural responses so as to minimize prediction errors across the hierarchy. Learning is thought to optimize the same objective with respect to the weights of synaptic connections. 

To demonstrate the meaning of the predictive coding objective, assume our visual system is composed of only one level of neurons together with a sensory input level. Let $x_t$ be the sensory input at time $t$ and let $z_t$ be the elicited neural responses. We assume the likelihood distribution, $p(x_t|z_t)$, is a Gaussian with mean $f(Wz_t)$, where $W$ is a weight matrix and $f$ is some non-linearity. We can also assume the co-variance of this Gaussian is the identity matrix for simplicity. The goal of predictive coding is to infer $z_t$ given $x_t$ and, over a longer time scale, learn the parameters in $W$. In their original paper, Rao and Ballard achieve this by directly minimizing the objective 
\begin{equation}
    \|f(Wz_t) - x_t\|_2^2 + \|z_t\|_2^2
\end{equation}
This optimization is done through gradient descent for each input sample $x_t$. For inference, the objective is minimized with respect to $z_t$, while it is minimized with respect to $W$ for learning at a slower time scale. This objective arises from maximizing the posterior probability $p(z_t|x_t)$ with the assumption that the prior distribution over $z_t$ is Gaussian. We can, therefore, think of the first term in the objective, which comes from the posterior, as the prediction error (or reconstruction loss) and the second term, which comes from the prior, as a regularization term which ensures that the inferred responses do not deviate too much from the model's prior biases. 

\subsection{Variational Autoencoders}
We can achieve the same objective of maximizing the posterior $p(z_t|x_t)$ by employing the technique of variation inference \cite{jordan_variational_methods}. By introducing an approximate \textit{variational} posterior $q(z_t|x_t)$, we can form the following lower bound on $\log{p(x_t)}$
\begin{equation}
    \log{p(x_t)} \geq \mathbb{E}_{z_t\sim q}[\log{p(x_t|z_t)}] - D_{KL}(q(z_t|x_t)||p(z_t))
\end{equation}
    
This lower bound is known as the evidence lower bound, or ELBO. When we assume the likelihood model, $p(x_t|z_t)$, to be Gaussian, the first term in the ELBO corresponds to the (negative) reconstruction loss. The second term represents the KL divergence between the inferred posterior distribution and the prior distribution over neural responses. Maximizing this objective, therefore, achieves the same purpose as the predictive coding objective. When we use neural networks to amortize this inference process, we end up with a variational autoencoder (VAE) \cite{kingma_vae}. We can therefore translate the theoretical neuroscience framework of predictive coding to deep learning using variational autoencoders.

==> conclusion.tex <==
We developed a novel, biologically-inspired model of active sensing by combining two theories from neuroscience: predictive coding for perception and uncertainty minimization for action. While these two theories have been utilized previously, our model incorporates them in a unique, scalable, and end-to-end framework, enabling flexible intrinsically-driven exploration for embodied AI. Furthermore, the proposed model provides an approximate method for learning policies that optimize information gain in a differentiable manner, utilizing a deep generative model. We test this model in two sensorimotor tasks that integrate perception and action: 1) learning transition dynamics through pure exploration in discrete environments, and 2) learning unsupervised representations in active vision. Remarkably, our model which is driven entirely in an intrinsic manner without extrinsic task-driven objectives as in animals exploring the world, discovers efficient action selections and sensorimotor representations, giving us insight into possible computational strategies employed by the brain.

